Network Newton-Part I: Algorithm and Convergence

We study the problem of minimizing a sum of convex objective functions where the components of the objective are available at different nodes of a network and nodes are allowed to only communicate with their neighbors. The use of distributed gradient methods is a common approach to solve this problem. Their popularity notwithstanding, these methods exhibit slow convergence and a consequent large number of communications between nodes to approach the optimal argument because they rely on first order information only. This paper proposes the network Newton (NN) method as a distributed algorithm that incorporates second order information. This is done via distributed implementation of approximations of a suitably chosen Newton step. The approximations are obtained by truncation of the Newton step's Taylor expansion. This leads to a family of methods defined by the number $K$ of Taylor series terms kept in the approximation. When keeping $K$ terms of the Taylor series, the method is called NN-$K$ and can be implemented through the aggregation of information in $K$-hop neighborhoods. Convergence to a point close to the optimal argument at a rate that is at least linear is proven and the existence of a tradeoff between convergence time and the distance to the optimal argument is shown. Convergence rate, several practical implementation matters, and numerical analyses are presented in a companion paper [3].

==> Simulations.tex <==
%!TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Numerical analysis}\label{sec:simulations}
 
We compare the performance of DGD and different versions of NN in the minimization of a distributed quadratic objective. The comparison is done in terms of both, number of iterations and number of information exchanges. Specifically, for each agent $i$ we consider a positive definite diagonal matrix $\bbA_i\in \mbS_{p}^{++}$ and a vector $\bbb_i \in \mbR^{p}$ to define the local objective function $f_i(\bbx)  :=  ({1}/{2}) \bbx^{T} \bbA_i\bbx +\bbb_i^T\bbx$. Therefore, the global cost function $f(\bbx)$ is written as
% 
\begin{equation}\label{example_problem}
  f(\bbx)  := \sum_{i=1}^n  \frac{1}{2} \bbx^{T} \bbA_i \bbx +\bbb_i^{T}\bbx   \ .
\end{equation}
%
The difficulty of solving \eqref{example_problem} is given by the condition number of the matrices $\bbA_i$. To adjust condition numbers we generate diagonal matrices $\bbA_i$ with random diagonal elements $a_{ii}$. The first $p/2$ diagonal elements $a_{ii}$ are drawn uniformly at random from the discrete set $\{1, 10^{-1},\ldots, 10^{-\xi}\}$ and the next $p/2$ are uniformly and randomly chosen from the set  $\{1,10^1,\ldots, 10^{\xi}\}$. This choice of coefficients yields local matrices $\bbA_i$ with eigenvalues in the interval $[10^{-\xi}, 10^{\xi}]$ and global matrices $\sum_{i=1}^{n}\bbA_i$ with eigenvalues in the interval $[n10^{-\xi}, n10^{\xi}]$. The condition numbers are typically $10^{2\xi}$ for the local functions and $10^\xi$ for the global objectives. The linear terms $\bbb_i^{T}\bbx$ are added so that the different local functions have different minima. The vectors $\bbb_i$ are chosen uniformly at random from the box $[0,1]^p$. 

For the quadratic objective in \eqref{example_problem} we can compute the optimal argument $\bbx^*$ in closed form. We then evaluate convergence through the relative error that we define as the average normalized squared distance between local vectors $\bbx_i$ and the optimal decision vector $\bbx^*$,
%%
\begin{equation}\label{distance_error}
e_t := \frac{1}{n} \sum_{i=1}^{n}\frac{\| \bbx_{i,t}-\bbx^*\|^2}{\|\bbx^*\|^2}.
\end{equation}
%
The network connecting the nodes is a $d$-regular cycle where each node is connected to exactly $d$ neighbors and $d$ is assumed even. The graph is generated by creating a cycle and then connecting each node with the $d/2$ nodes that are closest in each direction. The diagonal weights in the matrix $\bbW$ are set to $w_{ii} = 1/2+1/2(d+1)$ and the off diagonal weights to $w_{ij}= 1/2(d+1)$ when $j\in\ccalN_i$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{final_iteration_illustration.eps}
\caption{Convergence of DGD, NN-0, NN-1, and NN-2 in terms of number of iterations. The NN methods converges faster than DGD. Furthermore, the larger $K$ is, the faster NN-$K$ converges.}
\label{fig:iter_illus}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In the subsequent experiments we set the network size to $n=100$, the dimension of the decision vectors to $p=4$, the condition number parameter to $\xi=2$, the penalty coefficient inverse to $\alpha =10^{-2}$, and the network degree to $d=4$. The NN step size is set to $\eps=1$, which is always possible when we have quadratic objectives  [cf. Remark \ref{rmk_quadratic_obj}]. Figure \ref{fig:iter_illus} illustrates a sample convergence path for DGD, NN-0, NN-1, and NN-2 by measuring the relative error $e_t$ in \eqref{distance_error} with respect to the number of iterations $t$. As expected for a problem that doesn't have a small condition number -- in this particular instantiation of the function in \eqref{example_problem} the condition number is $95.2$ -- different versions of NN are much faster than DGD. E.g., after $t=1.5\times 10^3$ iterations the error associated which DGD iterates is $e_t\approx1.9\times 10^{-1}$. Comparable or better accuracy $e_t<1.9\times 10^{-1}$ is achieved in $t=132$, $t=63$, and $t=43$ iterations for NN-0, NN-1, and NN-2, respectively. 

Further recall that $\alpha$ controls the difference between the actual optimal argument  $\tby^*=[\bbx^*;\ldots;\bbx^*]$ [cf. \eqref{original_optimization_new_notation}] and the argument $\bby^*$ [cf. \eqref{centralized_opt_problem}] to which DGD and NN converge. Since we have $\alpha =10^{-2}$ and the difference between these two vectors is of order $O(\alpha)$, we expect the error in \eqref{distance_error} to settle at $e_t\approx10^{-2}$. The error actually settles at $e_t\approx6.3\times 10^{-3}$ and it takes all three versions of NN less than $t=400$ iterations to do so. It takes DGD more than $t=10^4$ iterations to reach this value. This relative performance difference decreases if the problem has better conditioning but can be made arbitrarily large by increasing the condition number of the matrix $\sum_{i=1}^{n}\bbA_i$. The number of iterations required for convergence can be further decreased by considering higher order approximations in \eqref{Hessian_approximation_iteration}. The advantages would be misleading because they come at the cost of increasing the number of communications required to approximate the Newton step.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{final-illustration.eps}
\caption{Convergence of DGD, NN-0, NN-1, and NN-2 in terms of number of communication exchanges. The NN-$K$ methods retain the advantage over DGD but increasing $K$ may not result in faster convergence. For this particular instance it is actually NN-1 that converges fastest in terms of number of communication exchanges. }
\label{fig:local_exch_illus}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
To study this latter effect we consider the relative performance of DGD and different versions of NN in terms of the number of local information exchanges. As pointed out in Remark \ref{rmk_comm_cost}, each iteration in NN-$K$ requires a total of $K+1$ information exchanges with each neighbor, as opposed to the single variable exchange required by DGD. After $t$ iterations the number of variable exchanges between each pair of neighbors is $t$ for DGD and $(K+1)t$ for NN-$K$. Thus, we can translate Figure \ref{fig:iter_illus} into a path in terms of number of communications by scaling the time axis by $(K+1)$. The result of this scaling is shown in Figure \ref{fig:local_exch_illus}. The different versions of NN retain a significant, albeit smaller, advantage with respect to DGD. Error $e_t<10^{-2}$ is achieved by NN-0, NN-1, and NN-2 after $(K+1)t=3.7\times 10^2$, $(K+1)t=3.1\times 10^2$, and $(K+1)t=3.4\times 10^2$ variable exchanges, respectively. When measured in this metric it is no longer true that increasing $K$ results in faster convergence. For this particular problem instance it is actually NN-1 that converges fastest in terms of number of communication exchanges. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{finalplot.eps}\vspace{-2mm}
\caption{Histograms of the number of information exchanges required to achieving accuracy $e_t<10^{-2}$. The qualitative observations made in figures \ref{fig:iter_illus} and \ref{fig:local_exch_illus} hold over a range of random problem realizations.}
\label{fig:local_exch_dist}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
For a more more comprehensive evaluation we consider $10^3$ different random realizations of \eqref{example_problem} where we also randomize the degree $d$ of the $d$-regular graph that we choose from the even numbers in the set $[2,10]$. The remaining parameters are the same used to generate figures \ref{fig:iter_illus} and \ref{fig:local_exch_illus}. For each joint random realization of network and objective we run DGD, NN-0, NN-1, and NN-2, until achieving error $e_t<10^{-2}$ and record the number of communication exchanges that have elapsed -- which amount to simply $t$ for DGD and $(K+1)t$ for NN. The resulting histograms are shown in Figure \ref{fig:local_exch_dist}. The mean times required to reduce the error to $e_t<10^{-2}$ are $4.3\times 10^3$ for DGD and $4.0\times 10^2$, $3.5\times 10^2$, and $3.7\times 10^2$ for NN-0, NN-1, and NN-2. As in the particular case shown in figures \ref{fig:iter_illus} and \ref{fig:local_exch_illus}, NN-1 performs best in terms of communication exchanges. Observe, however, that the number of communication exchanges required by NN-2 is not much larger and that NN-2 requires less computational effort than NN-1 because the number of iterations $t$ is smaller. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{all_alpha_1e-2.eps}
\caption{{Convergence of adaptive DGD, NN-0, NN-1, and NN-2 for $\alpha_0=10^{-2}$. NN methods require less iterations than DGD.}}
\label{fig:4_2}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{all_alpha_1e-1.eps}
\caption{{Convergence of Adaptive DGD, NN-0, NN-1, and NN-2 for $\alpha_0=10^{-1}$. ANN methods require less iterations than DGD and convergence of all algorithms are faster relative to the case that $\alpha_0=10^{-2}$.}}
\label{fig:4}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Adaptive Network Newton}\label{sec_sims_ann}

Given that DGD and NN are penalty methods it is of interest to consider their behavior when the inverse penalty parameter $\alpha$ is decreased recursively. The adaptation of $\alpha$ for NN-$K$ is discussed in Section \ref{sec:implement} where it is termed adaptive (A)NN-$K$. The same adaptation strategy is considered here for DGD. The parameter $\alpha$ is kept constant until the local gradient components $\bbg_{i,t}$ become smaller than a given tolerance $\text{tol}$, i.e., until $\|\bbg_{i,t}\|\leq \text{tol}$ for all $i$. When this tolerance is achieved, the parameter $\alpha$ is scaled by a factor $\eta<1$, i.e., $\alpha$ is decreased from its current value to $\eta\alpha$. This requires the use of a signaling method like the one summarized in Algorithm \ref{algo_ANN} for ANN-$K$.

We consider the objective in \eqref{example_problem} and nodes connected by a $d$-regular cycle. We use the same parameters used to generate figures \ref{fig:iter_illus} and \ref{fig:local_exch_illus}. The adaptive gradient tolerance is set to $\text{tol}=10^{-3}$ and the scaling parameter to $\eta=10$. We consider two different scenarios where the initial penalty parameters are $\alpha=\alpha_{0}=10^{-1}$ and $\alpha=\alpha_0=10^{-2}$. The respective error trajectories $e_t$ with respect to the number o iterations are shown in figures \ref{fig:4_2} -- where  $\alpha_0=10^{-2}$ -- and \ref{fig:4} -- where $\alpha_0=10^{-1}$. In each figure we show $e_t$ for adaptive DGD, ANN-0, ANN-1, and ANN-2. Both figures show that the ANN methods outperform adaptive DGD and that larger $K$ reduces the number of iterations that it takes ANN-$K$ to achieve a target error. These results are consistent with the findings summarized in figures \ref{fig:iter_illus}-\ref{fig:local_exch_dist}. 

More interesting conclusions follow from a comparison across figures \ref{fig:iter_illus} and \ref{fig:local_exch_illus}. We can see that it is better to start with the (larger) value $\alpha=10^{-1}$ even if the method initially converges to a point farther from the actually optimum. This happens because problems with larger $\alpha$ are better conditioned and thus easier to minimize.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{separable_data_1.eps}
\caption{{Convergence of DGD, NN-0, NN-1, and NN-2. NN methods for a linearly separable logistic regression.}}
\label{fig:5}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.63\linewidth]{separable_noisy_data_1.eps}
\caption{{Convergence of DGD, NN-0, NN-1, and NN-2. NN methods for a non-linearly separable logistic regression.}}
\label{fig:43}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Logistic regression}

For a more realistic test we consider the application of NN for solving a logistic regression problem. In this problem we are given $q$ training samples that we distribute across $n$ distinct servers. Denote as $q_i$ the number of samples that are assigned to server $i$. Each of the training samples at node $i$ contains a feature vector $\bbu_{il}\in \reals^p$ and a class $v_{il}\in \{-1,1\}$. The goal is to predict the probability  $\Pc{v=1\mid \bbu}$ of having label $v=1$ when given a feature vector $\bbu$ whose class is not known. The logistic regression model assumes that this probability can be computed as $\Pc{v=1\mid \bbu}=1/(1+\exp(-\bbu^T\bbx))$ for a linear classifier $\bbx$ that is computed based on the training samples. It follows from this model that the regularized maximum log likelihood estimate of the classifier $\bbx$ given the training samples $(\bbu_{il},v_{il})$ for $l=1,\ldots,q_i$ and $i=1,\ldots, n$ is given by
%
\begin{align}\label{eqn_logistic_regrssion_max_likelihood}
   \bbx^*\  =\ &   \argmin_\bbx f(\bbx) \\ \nonumber
         \ :=\ &   \argmin_\bbx   \frac{\lambda}{2} \|\bbx\|^2 
             +               \sum_{i=1}^n \sum_{l=1}^{q_i} 
                                  \log \Big[1+\exp(-v_{il}\bbu_{il}^T\bbx)\Big],
\end{align}
%
where we defined the function $f(\bbx)$ for future reference. The regularization term $(\lambda/2)\|\bbx\|^2$ is added to reduce overfitting to the training set. 

The optimization problem in \eqref{eqn_logistic_regrssion_max_likelihood} can be written in the form of the optimization problem in \eqref{original_optimization_problem1}. To do so simply define the local objective functions $f_i$ as 
%
\begin{equation}
   f_i(\bbx) =    \frac{\lambda}{2n} \|\bbx\|^2
                + \sum_{l=1}^{q_i} \log \Big[1+\exp(-v_{il}\bbu_{il}^T\bbx)\Big],
\end{equation}
%
and observe that given this definition we can write the objective in \eqref{eqn_logistic_regrssion_max_likelihood} as $f(\bbx)=\sum_{i=1}^n f_i(\bbx)$. We can then solve \eqref{eqn_logistic_regrssion_max_likelihood} in a distributed manner using DGD and NN-$K$ methods. 

In our experiments we use a synthetic dataset where each component of the feature vector $\bbu_{{il}}$ with label $v_{il}=1$ is generated from a normal distribution with mean $\mu$ and standard deviation $\sigma_+$, while sample points with label $v_{il}=-1$ are generated with mean $-\mu$ and standard deviation $\sigma_-$. The network is a $d$-regular cycle. The diagonal weights in the matrix $\bbW$ are set to $w_{ii} = 1/2+1/2(d+1)$ and the off diagonal weights to $w_{ij}= 1/2(d+1)$ when $j\in\ccalN_i$. We set the feature vector dimension to $p=10$, the number of training samples per node at $q_i=50$, and the regularization parameter to $\lambda=10^{-4}$. The number of nodes is $n=100$ and the degree of the $d$-regular cycle is $d=4$.

We consider first a scenario in which the dataset is linearly separable. To generate a linearly separable dataset the mean is set to $\mu=3$ and the standard deviations to 
$\sigma_+=\sigma_-=1$. Figure \ref{fig:5} illustrates the convergence path of the objective function $F(\bby)$ [cf. \eqref{centralized_opt_problem}] when the penalty parameter is $\alpha=10^{-2}$ and the NN step size is $\eps=1$. The reduction in the number of iterations required to achieve convergence is a little more marked than in the quadratic example considered in figures \ref{fig:iter_illus}-\ref{fig:local_exch_dist}. The objective function values $F(\bby_t)$ for NN-0, NN-1 and NN-2 after $t=500$ iterations are below $1.6\times 10^{-4}$, while for DGD the objective function value after the same number of iterations have passed is $F(\bby_t)=2.6\times 10^{-3}$. Conversely, achieving accuracy $F(\bby_t)=2.6\times 10^{-3}$ for NN-0, NN-1, and NN-2 requires $68$, $33$, and $19$ iterations, respectively, while DGD requires $500$ iterations. Observe that for this example NN-2 performs better than NN-1 and NN-0 not only in the number of iterations but also in the number of variable exchanges required to achieve a target accuracy.

We also consider a case in which the dataset is {\it not} linearly separable. To generate this dataset we set the mean to $\mu=2$ and the standard deviations to $\sigma_+=\sigma_-=2$. The penalty parameter is set to $\alpha=10^{-2}$ and the NN step size to $\eps=1$. The resulting objective trajectories $F(\bby_t)$ of DGD, NN-0, NN-1, and NN-2 are shown in Figure \ref{fig:43}. The advantages of the NN methods relative to DGD are less pronounced but still significant. In this case we also observe that  NN-2 performs best in terms of number of iterations and number of communication exchanges.






